Sensitivity Analysis of Error-Contaminated Time Series Data under Autoregressive Models with Application of COVID-19 Data

Autoregressive (AR) models are useful tools in time series analysis. Inferences under such models are distorted in the presence of measurement error, which is very common in practice. In this article, we establish analytical results for quantifying the biases of the parameter estimation in AR models if the measurement error effects are neglected. We propose two measurement error models to describe different processes of data contamination. An estimating equation approach is proposed for the estimation of the model parameters with measurement error effects accounted for. We further discuss forecasting using the proposed method. Our work is inspired by COVID-19 data, which are error-contaminated due to multiple reasons including the asymptomatic cases and varying incubation periods. We implement our proposed method by conducting sensitivity analyses and forecasting of the mortality rate of COVID-19 over time for the four most populated provinces in Canada. The results suggest that incorporating or not incorporating measurement error effects yields rather different results for parameter estimation and forecasting.

==> maintextv1.tex <==
%----------------------------------------------------------------------------------------
%	INTRODUCTION
%----------------------------------------------------------------------------------------

\section{Introduction (Working)} % Major section

% ------------------------------------------------


%----------------------------------------------------------------------------------------
%	MAJOR SECTION 1
%----------------------------------------------------------------------------------------

\section{Model Setup and Framework} \label{Sec:Setup}% Major section
%------------------------------------------------
\subsection{Time Series Model for Count Data}

Consider a $T\times 1$ vector of time series of non-negative counts,  $Y^{(T)}=(Y_1,Y_2, \ldots, Y_T)^{\rm \scalebox{0.6}{T}}$. for $t=1,\ldots,
T$, let $\mu_{t|t-1} = E(Y_t|Y^{(t-1)})$ be the conditional mean of $Y_t$ given its previous observations. Assume that $Y_t$ given $Y^{(t-1)}$ follows a Poisson distribution with mean $\mu_{t|t-1}$. Namely, the conditional probability function of $Y_{t}$, given $Y^{(t-1)}=y^{(t-1)}$, is
\begin{equation}\label{eqn:pdfYt}
    P(Y_t=y_t|Y^{(t-1)}=y^{(t-1)}) = \frac{\mu_{t|t-1}^{y_t}}{y_t!} e^{-\mu_{t|t-1}} \qquad \text{ for } y_t=0,1,\cdots.
\end{equation}

We are interested in modeling the dependence of $\mu_{t|t-1}$ on $Y^{(t-1)}$ and we consider it to be postulated the log linear autoregressive  time series model with $p$-lags
\begin{equation}\label{eqn:timeseriresmodel}
    \log \ \mu_{t|t-1} =  \beta_0 + \sum_{j=1}^p \beta_j y_{t-j},
\end{equation}
where $\beta_p=(\beta_0,\ldots,\beta_p)^{\rm \scalebox{0.6}{T}}$ is the parameter to be estimated.


%The specification of model~\ref{\label{eqn:timeseriresmodel}} is observation-driven, which is in contrast to the parameter-driven model. 

We comment that when $\beta$ are all positive, the model is explosive because $\beta_jy_{t-j}$ is non-negative for $j=1,\ldots,p$. To avoid the explosive problem, a variation is proposed by \citet{zeger1988markov} to replace $y_{t-j}$ in (\ref{eqn:timeseriresmodel}) by  $\log \  y_{t-j}$.
To highlight the key ideas, without using complicated expressions, in the following development we take $p=1$.



\subsection{Measurement Error Models}

Suppose that for $t=1,\ldots,T$ the observation of $Y_t$ is subject to measurement error  and the precise measurement of $Y_t$ may not be observed, while its surrogate measurement $Y_t^*$ is available. Let $Z_{t}=(z_{t1},\ldots,z_{tq})^{\rm \scalebox{0.6}{T}}$ denote the covariates vector that is related to the measurement error process. We assume that given the true observations $Y_{t}$, the observed surrogates $Y_{t}^*$ are independent for $t=1,\ldots,T$, with
\begin{equation}\label{eqn:assumption1}
    f(y_{1}^*,\ldots,y_{T}^*|y_{1},\ldots,y_{T}) = \prod_{t=1}^T f(y_{t}^*|y_t),
\end{equation}
where $f(\cdot|\cdot)$ represents the conditional probability mass function for the variables indicated by the arguments. We also assume that $Y_t^*$ is less or equal to $Y_t$.

We consider two different measurement error models. The first measurement error model is
\begin{equation}\label{eqn:measmodelClassic}
    Y_t^* = Y_{t} - e_t,
\end{equation}
where the error term $e_t$ depends on $Y_t$, and conditional on $Y_t=y_t$, $e_t$ follows a Binomial$(y_t,\pi_t)$ with $\pi_t$ being the parameter between 0 and 1. 

Furthermore, we use a regression model to facilitate the possible dependence of $\pi_t$ on $Z_{t}$,
\begin{equation}\label{eqn:measmodelpi}
    g(\pi_t) = \alpha^{\rm \scalebox{0.6}{T}}Z_{t},
\end{equation}
where $\alpha$ is the regression parameter, and $g(\cdot)$ is the link function. Common choices of $g(x)$ include the logit link $g(x) = \log \frac{1}{1-x}$, the probit link $g(x)= \Phi^{-1}(x)$, and the complementary log-log link $g(x)=\log\{-\log(1-x)\}$ where $\phi(\cdot)$ is the cumulative distribution function of the standard normal distribution.

The second model is the Berkson-like model
\begin{equation}
    Y_{t} = Y_{t}^* + \epsilon_t,
\end{equation}
where the error term $\epsilon_t$ is independent of $Y_t^*$, and $\epsilon_t$ follows a Poisson distribution with mean $\lambda_t$. The modeling of the dependence of $\lambda_t$ on covariates can be accommodated by the generalized linear model
\begin{equation}
    g(\lambda_t) = \alpha^{\rm \scalebox{0.6}{T}}Z_{t},
\end{equation}
where $g(x)= \log \ x$ is the log link, and $\alpha$ is the regression parameter.                                                                                                                                                                                                             

\section{Methodology}

The parameter $\beta$ in the time series model and parameter $\alpha$ can be estimated through maximum likelihood method. We first derive the likelihood function
\begin{align}
    L_T(y;\beta,\alpha) &= \sum_{y_{1}} \cdots \sum_{y_{T}} f(y_{1}^*,\ldots,y_{p}^*|y_{1},\ldots,y_{p})f(y_{1},\ldots,y_{p})  \\
    &= \sum_{y_{1}} \cdots \sum_{y_{T}} f(y_1)\prod_{t=2}^T f(y_t^*|y_t) f(y_t|y_{t-1}) d\,y_{1}\ldots d\,y_{p}, \label{eqn:likeli}
\end{align}
where (\ref{eqn:likeli}) is due to the assumption (\ref{eqn:assumption1}). 

Let $\theta=(\beta^{\rm \scalebox{0.6}{T}},\alpha^{\rm \scalebox{0.6}{T}})^{\rm \scalebox{0.6}{T}}$. The estimation of parameter $\theta$ can be carried out by maximizing the likelihood (\ref{eqn:likeli}), which is equivalent to solving the equation
\begin{equation}
    S_T(\theta) = 
    \frac{\partial  \log\, L_T(y; \theta) }{\partial \theta} = 0,
\end{equation}
which gives the estimators, say $\widehat{\theta}$, of $\theta$.


Under regularity conditions \citep{jensen1999asymptotic}, $\hat{\theta}$ is a consistent estimator of $\theta$, and 
\begin{equation*}
    \sqrt{T} (\hat{\theta}-\theta) \xrightarrow{\ d \ } N(0,J_0(\theta)) \qquad \text{as} \qquad T\xrightarrow{}\infty
\end{equation*}
where  $J_0(\theta)$ is the fisher information matrix given by the limiting covariance matrix of $\frac{1}{T}S_T(\theta)$, which is also given by
\begin{equation*}
    J_0(\theta) = E(\eta\eta^{\rm \scalebox{0.6}{T}}),
\end{equation*}
where $\eta = \lim_{t\to\infty} \frac{\partial }{\partial \theta} \log f(Y_t^*|Y_{t-1}^*,\ldots,Y_1^*)$.


% Under regularity conditions, $\hat{\theta}$ is a consistent estimator of $\theta$, and 
% \begin{equation*}
%     \sqrt{n} (\hat{\theta}-\theta) \xrightarrow{d} N(0,I^{-1}(\theta)) \qquad \text{as} \qquad n\xrightarrow{}\infty
% \end{equation*}
% where 
% \begin{equation}\label{eqn:fisherinfo}
% I(\theta)=E\left\{S_i(\theta)S_i^{\rm \scalebox{0.6}{T}}(\theta)\right\}.
% \end{equation}

\section{Application to Novel Coronavirus Data} \label{sec:dataanalysis}

\section{Simulations}

\section{Discussion}

==> tables/ADFtest2.tex <==
% \begin{table}[htbp]
% \centering
% \caption{The result of the Dickey-Fuller test \label{tab:ADFtest}}
% \begin{tabular}{lcclcc}
% \hline
%                                     & \multicolumn{2}{c}{Confirmed Case} &  & \multicolumn{2}{c}{Death} \\ \cline{2-3} \cline{5-6} 
%                                     & ADF             & p-value          &  & ADF         & p-value     \\ \hline
% Logarithm                           & 0.666           & 0.99             &  & -2.83       & 0.07       \\
% Logarithm and 1-lag differentiation & -8.27           & $<$0.01          &  & -10.53      & $<$0.01     \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\centering
\caption{The result of the Dickey-Fuller test \label{tab:ADFtest2}}
\begin{tabular}{lccccc}
\hline
                                    & \multicolumn{2}{c}{British Columbia} &  & \multicolumn{2}{c}{Ontario} \\ \cline{2-3} \cline{5-6} 
                                    & ADF              & p-value           &  & ADF         & p-value       \\ \hline
No transformation                           & -3.23             & 0.010            &  & -3.16       & 0.037        \\ \hline
\end{tabular}
\end{table}

==> tables/Table_Canada.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model under different degree of measurement error}\label{tab:TableCanada}
\begin{tabular}{cccccccccc}
\hline
\multicolumn{1}{l}{}            & \multicolumn{1}{l}{}         &           & \multicolumn{3}{c}{British Columbia} &  & \multicolumn{3}{c}{Ontario} \\ \cline{1-6} \cline{8-10} 
Model                           & Degree                       & Parameter & EST        & s.d.      & p-value     &  & EST     & s.d.   & p-value  \\ \hline
\multirow{3}{*}{Naive}          & \multirow{3}{*}{-}           & $\phi_0$  & 0.406      & 0.148     & 0.018       &  & 0.970   & 0.128  & 0.000    \\
                                &                              & $\phi_1$  & -0.226     & 0.159     & 0.180       &  & 0.025   & 0.100  & 0.804    \\
                                &                              & $\phi_2$  & 0.376      & 0.131     & 0.014       &  & 0.263   & 0.049  & <0.001    \\ \hline
\multirow{6}{*}{Additive}       & \multirow{3}{*}{Mild}        & $\phi_0$  & 0.217      & 0.084     & 0.024       &  & 0.521   & 0.111  & 0.000    \\
                                &                              & $\phi_1$  & -0.231     & 0.167     & 0.192       &  & 0.030   & 0.185  & 0.874    \\
                                &                              & $\phi_2$  & 0.390      & 0.152     & 0.024       &  & 0.223   & 0.050  & <0.001    \\ \cline{2-10} 
                                & \multirow{3}{*}{Substantial} & $\phi_0$  & 0.163      & 0.280     & 0.572       &  & 0.503   & 0.413  & 0.235    \\
                                &                              & $\phi_1$  & -0.233     & 0.627     & 0.716       &  & 0.064   & 0.756  & 0.933    \\
                                &                              & $\phi_2$  & 0.600      & 0.490     & 0.244       &  & 0.103   & 0.051  & 0.052    \\ \hline
\multirow{6}{*}{Multiplicative} & \multirow{3}{*}{Mild}        & $\phi_0$  & 0.217      & 0.084     & 0.025       &  & 0.522   & 0.098  & 0.000    \\
                                &                              & $\phi_1$  & -0.231     & 0.169     & 0.198       &  & 0.029   & 0.157  & 0.854    \\
                                &                              & $\phi_2$  & 0.391      & 0.148     & 0.021       &  & 0.066   & 0.014  & <0.001    \\ \cline{2-10} 
                                & \multirow{3}{*}{Substantial} & $\phi_0$  & 0.206      & 0.107     & 0.078       &  & 0.508   & 0.731  & 0.493    \\
                                &                              & $\phi_1$  & -0.242     & 0.210     & 0.272       &  & 0.054   & 1.377  & 0.969    \\
                                &                              & $\phi_2$  & 0.443      & 0.197     & 0.044       &  & 0.036   & 0.016  & 0.032    \\ \hline
\end{tabular}
\end{table}

==> tables/Table_Peh.tex <==
\begin{sidewaystable}
\setlength\extrarowheight{1pt} % provide a bit more vertical whitespace
\centering
\captionsetup{size=small}
\tiny

\begin{threeparttable}
\caption[]{The observed prediction error and expected prediction error for different lag order of autoregressive models.}
\label{Tab:TablePeh}

\begin{tabular}{lllccccccccccccc}
\hline
                                &                                &                                            & \multicolumn{6}{c}{Observed Prediction Error}                                          &  & \multicolumn{6}{c}{Expected Prediction Error}                      \\ \hline
Method                          & $\sigma_e^2$ (or $\sigma_u^2$) & Model                                      & Day 1                     & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm OPE}(h)$ &  & Day 1 & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm EPE}(h)$ \\ \cline{1-9} \cline{11-16} 
                                &                                & \multicolumn{7}{l}{British Columbia}                                                                                                &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(1)}} & \multicolumn{1}{l}{0.053} & 0.037 & 0.105 & 0.148 & 0.079 & 0.421                      &  & 0.207 & 0.234 & 0.237 & 0.238 & 0.238 & 1.153                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.029 & 0.004 & 0.046                      &  & 0.196 & 0.223 & 0.227 & 0.228 & 0.228 & 1.101                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.004                     & 0.000 & 0.009 & 0.028 & 0.004 & 0.045                      &  & 0.106 & 0.134 & 0.143 & 0.146 & 0.147 & 0.676                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.029 & 0.004 & 0.046                      &  & 0.057 & 0.065 & 0.066 & 0.066 & 0.066 & 0.321                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.028 & 0.004 & 0.046                      &  & 0.049 & 0.056 & 0.058 & 0.058 & 0.058 & 0.278                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{\textbf{AR(2)}\tnote{a}}            & 0.025                     & 0.082 & 0.110 & 0.146 & 0.074 & 0.437                      &  & 0.177 & 0.186 & 0.219 & 0.225 & 0.232 & 1.039                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.001                     & 0.001 & 0.008 & 0.027 & 0.003 & 0.040                      &  & 0.166 & 0.175 & 0.207 & 0.213 & 0.221 & 0.981                      \\
                                & Moderate                       &                                            & 0.001                     & 0.001 & 0.010 & 0.028 & 0.003 & 0.044                      &  & 0.064 & 0.067 & 0.093 & 0.098 & 0.111 & 0.433                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.001                     & 0.001 & 0.008 & 0.027 & 0.003 & 0.040                      &  & 0.049 & 0.051 & 0.060 & 0.062 & 0.064 & 0.287                      \\
                                & Moderate                       &                                            & 0.001                     & 0.001 & 0.009 & 0.026 & 0.003 & 0.040                      &  & 0.039 & 0.041 & 0.050 & 0.052 & 0.054 & 0.235                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{AR(3)}                     & 0.000                     & 0.054 & 0.103 & 0.198 & 0.086 & 0.442                      &  & 0.168 & 0.184 & 0.185 & 0.186 & 0.187 & 0.910                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.028                     & 0.003 & 0.005 & 0.047 & 0.002 & 0.086                      &  & 0.156 & 0.172 & 0.172 & 0.173 & 0.175 & 0.848                      \\
                                & Moderate                       &                                            & 0.055                     & 0.002 & 0.001 & 0.068 & 0.003 & 0.129                      &  & 0.064 & 0.089 & 0.128 & 0.203 & 0.301 & 0.784                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.028                     & 0.003 & 0.005 & 0.047 & 0.002 & 0.086                      &  & 0.046 & 0.051 & 0.051 & 0.051 & 0.051 & 0.249                      \\
                                & Moderate                       &                                            & 0.034                     & 0.003 & 0.004 & 0.053 & 0.002 & 0.097                      &  & 0.039 & 0.044 & 0.043 & 0.042 & 0.042 & 0.210                      \\ \hline
                                &                                & \multicolumn{7}{l}{Ontario}                                                                                                         &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multirow{5}{*}{\textbf{AR(1)}\tnote{a}}            & 0.084                     & 0.097 & 0.177 & 0.070 & 0.039 & 0.467                      &  & 0.263 & 0.264 & 0.264 & 0.264 & 0.264 & 1.318                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.023                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.151                      &  & 0.223 & 0.224 & 0.224 & 0.224 & 0.224 & 1.118                      \\
                                & Moderate                       &                                            & 0.014                     & 0.020 & 0.001 & 0.037 & 0.068 & 0.141                      &  & 0.103 & 0.104 & 0.104 & 0.104 & 0.104 & 0.518                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.023                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.151                      &  & 0.066 & 0.066 & 0.066 & 0.066 & 0.066 & 0.331                      \\
                                & Moderate                       &                                            & 0.017                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.144                      &  & 0.036 & 0.036 & 0.036 & 0.036 & 0.036 & 0.179                      \\ \cline{3-16} 
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(2)}} & 0.038                     & 0.113 & 0.173 & 0.071 & 0.039 & 0.434                      &  & 0.259 & 0.259 & 0.263 & 0.263 & 0.264 & 1.308                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.111                     & 0.008 & 0.003 & 0.036 & 0.068 & 0.226                      &  & 0.218 & 0.218 & 0.223 & 0.223 & 0.224 & 1.107                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.264                     & 0.002 & 0.017 & 0.021 & 0.081 & 0.386                      &  & 0.094 & 0.095 & 0.102 & 0.103 & 0.103 & 0.498                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.109                     & 0.008 & 0.002 & 0.036 & 0.068 & 0.224                      &  & 0.065 & 0.065 & 0.066 & 0.066 & 0.066 & 0.329                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.212                     & 0.000 & 0.010 & 0.027 & 0.074 & 0.323                      &  & 0.036 & 0.036 & 0.036 & 0.036 & 0.036 & 0.180                      \\ \hline
\end{tabular}

\begin{tablenotes}
\item[a]{\scriptsize The selected model}
\end{tablenotes}


\end{threeparttable}
\end{sidewaystable}


==> tables/Table_alpha0.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model with different $\alpha_0$}\label{tab:Tablealpha0}
\begin{tabular}{lccccccccc}
\hline
                          & \multicolumn{1}{l}{}  &           & \multicolumn{3}{c}{Time Series 1}                   &  & \multicolumn{3}{c}{Time Series 2}                    \\ \cline{1-6} \cline{8-10} 
Model                     & $\alpha_0$            & Parameter & Point Estimation (s.d.) & p-value & CI              &  & Point Estimation (s.d.) & p-value & CI               \\ \hline
\multirow{2}{*}{Naive}    & -                     & $\phi_0$  & 0.440 (0.112)           & 0.002   & (0.197, 0.683)  &  & -0.144 (0.049)          & 0.005   & (-0.242, -0.046) \\
                          & -                     & $\phi_1$  & -0.286 (0.157)          & 0.093   & (-0.629, 0.056) &  & -0.271 (0.053)          & 0.000   & (-0.378, -0.163) \\ \hline
\multirow{8}{*}{Additive} & \multirow{2}{*}{0}    & $\phi_0$  & 0.458 (0.120)           & 0.002   & (0.196, 0.719)  &  & -0.148 (0.051)          & 0.006   & (-0.252, -0.044) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.098   & (-0.749, 0.073) &  & -0.303 (0.055)          & 0.000   & (-0.414, -0.192) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.01} & $\phi_0$  & 0.444 (0.117)           & 0.002   & (0.190, 0.699)  &  & -0.161 (0.050)          & 0.003   & (-0.262, -0.060) \\
                          &                       & $\phi_1$  & -0.338 (0.186)          & 0.095   & (-0.744, 0.068) &  & -0.303 (0.053)          & 0.000   & (-0.410, -0.195) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.05} & $\phi_0$  & 0.391 (0.111)           & 0.004   & (0.150, 0.632)  &  & -0.213 (0.049)          & 0.000   & (-0.312, -0.114) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.099   & (-0.749, 0.073) &  & -0.303 (0.054)          & 0.000   & (-0.412, -0.194) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.1}  & $\phi_0$  & 0.324 (0.104)           & 0.009   & (0.097, 0.551)  &  & -0.278 (0.048)          & 0.000   & (-0.375, -0.182) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.099   & (-0.749, 0.073) &  & -0.303 (0.054)          & 0.000   & (-0.412, -0.194) \\ \hline
\end{tabular}
\end{table}

==> tables/Table_sigmas.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model under different degree of measurement error}\label{tab:TableAR}
\begin{tabular}{llcccccccc}
\hline
                                &                              &           & \multicolumn{3}{c}{Time Series 1}             &  & \multicolumn{3}{c}{Time Series 2}              \\ \cline{4-6} \cline{8-10} 
Model                           & Degree                       & Parameter & Estimates (s.e.) & P-value  & CI              &  & Estimates (s.e.) & P-value  & CI               \\ \hline
\multirow{2}{*}{Naive}          & \multirow{2}{*}{-}           & $\phi_0$  & -0.144 (0.097)   & 0.163    & (-0.356, 0.067) &  & -0.144 (0.067)   & 0.036    & (-0.279, -0.010) \\
                                &                              & $\phi_1$  & -0.271 (0.155)   & 0.106    & (-0.608, 0.067) &  & -0.271 (0.064)   & $<$0.001 & (-0.399, -0.142) \\ \hline
\multirow{6}{*}{Additive}       & \multirow{2}{*}{Mild}        & $\phi_0$  & 0.422 (0.096)    & $<$0.001 & (0.212, 0.631)  &  & -0.145 (0.064)   & 0.030    & (-0.275, -0.015) \\
                                &                              & $\phi_1$  & -0.283 (0.154)   & 0.092    & (-0.620, 0.053) &  & -0.278 (0.068)   & $<$0.001 & (-0.416, -0.140) \\ \cline{3-10} 
                                & \multirow{2}{*}{Moderate}    & $\phi_0$  & 0.439 (0.103)    & $<$0.001 & (0.214, 0.664)  &  & -0.154 (0.069)   & 0.032    & (-0.294, -0.014) \\
                                &                              & $\phi_1$  & -0.335 (0.174)   & 0.078    & (-0.714, 0.044) &  & -0.355 (0.073)   & $<$0.001 & (-0.502, -0.209) \\ \cline{3-10} 
                                & \multirow{2}{*}{Substantial} & $\phi_0$  & 0.596 (0.350)    & 0.114    & (-0.166, 1.357) &  & -0.180 (0.159)   & 0.266    & (-0.502, 0.142)  \\
                                &                              & $\phi_1$  & -0.812 (1.070)   & 0.462    & (-3.145, 1.520) &  & -0.585 (0.954)   & 0.543    & (-2.512, 1.342)  \\ \hline
\multirow{6}{*}{Multiplicative} & \multirow{2}{*}{Mild}        & $\phi_0$  & 0.422 (0.098)    & $<$0.001 & (0.209, 0.636)  &  & -0.146 (0.066)   & 0.032    & (-0.278, -0.013) \\
                                &                              & $\phi_1$  & -0.284 (0.157)   & 0.096    & (-0.627, 0.058) &  & -0.282 (0.067)   & $<$0.001 & (-0.418, -0.146) \\ \cline{3-10} 
                                & \multirow{2}{*}{Moderate}    & $\phi_0$  & 0.458 (0.123)    & $<$0.001 & (0.189, 0.727)  &  & -0.160 (0.073)   & 0.034    & (-0.308, -0.012) \\
                                &                              & $\phi_1$  & -0.394 (0.225)   & 0.106    & (-0.884, 0.097) &  & -0.410 (0.095)   & $<$0.001 & (-0.602, -0.218) \\ \cline{3-10} 
                                & \multirow{2}{*}{Substantial} & $\phi_0$  & 0.635 (0.327)    & 0.076    & (-0.078, 1.348) &  & -0.184 (0.086)   & 0.039    & (-0.359, -0.010) \\
                                &                              & $\phi_1$  & -0.932 (0.716)   & 0.218    & (-2.493, 0.629) &  & -0.624 (0.138)   & $<$0.001 & (-0.902, -0.345) \\ \hline
\end{tabular}
\end{table}
